FedSelect: Personalized Federated Learning with Customized Selection of Parameters for Fine-Tuning

Standard federated learning approaches suffer when client data distributions have sufficient heterogeneity. Recent methods addressed the client data heterogeneity issue via personalized federated learning (PFL) - a class of FL algorithms aiming to personalize learned global knowledge to better suit the clients' local data distributions. Existing PFL methods usually decouple global updates in deep neural networks by performing personalization on particular layers (i.e. classifier heads) and global aggregation for the rest of the network. However, preselecting network layers for personalization may result in suboptimal storage of global knowledge. In this work, we propose FedSelect, a novel PFL algorithm inspired by the iterative subnetwork discovery procedure used for the Lottery Ticket Hypothesis. FedSelect incrementally expands subnetworks to personalize client parameters, concurrently conducting global aggregations on the remaining parameters. This approach enables the personalization of both client parameters and subnetwork structure during the training process. Finally, we show that FedSelect outperforms recent state-of-the-art PFL algorithms under challenging client data heterogeneity settings and demonstrates robustness to various real-world distributional shifts. Our code is available at https://github.com/lapisrocks/fedselect.

==> sec/1_intro.tex <==
\section{Introduction}

At present, learning tasks require a significant amount of training data for deep neural networks (DNNs) to perform effectively. Unfortunately, DNNs face two major challenges: the high cost of collecting data and the increasing concerns around privacy. These challenges can hinder the performance of DNNs, which are crucial for various applications such as image recognition, natural language processing, and speech recognition. This makes the creation of communication-efficient and privacy-preserving learning algorithms critical for utilizing data across client sources like data silos and mobile devices. Federated learning \cite{mcmahan2017, Li_2020} is the primary machine learning framework for this setting. It preserves data privacy during collaborative training by disseminating model updates from clients to a central server, instead of pooling raw data at one location. This approach allows for the learning process to leverage distributed data across numerous clients without directly sharing the data, thus preserving local data confidentiality and potentially enhancing model performance beyond what could be attained individually. Federated learning is particularly beneficial for privacy-critical applications, such as the analysis of medical data \citep{sheller2020federated}. However, a significant challenge in federated learning is the variability in data distribution across different clients, known as data heterogeneity. \as{I think we should write a few sentences on FL definition, the connection between clients and hub, communications, etc.}
\chulin{rewrite, 2-3 sentences are enough}


To address this issue, personalized federated learning (PFL) customizes client models to their unique data distributions. Common strategies involve \textit{full model personalization}, where each client trains both a local and a global model. This, however, doubles the computational demand compared to the standard federated learning approach and may not be feasible in settings where client memory and computational capability are limited \citep{dinh2020personalized,li2021ditto}. An alternative, \textit{partial model personalization}, divides the model into shared and client-specific parameters \citep{pillutla2022federated}, with only the shared parameters undergoing global updates. While this reduces computational load, it can lead to models that are too closely fitted to local data, degrading overall performance. Furthermore, the design of the personalized architecture is fixed prior to training and lacks adaptability to specific use cases.
\chulin{remove full model per.}

% WB: currently working on this paragraph





challenges 
why parameter-wise: more fine-grained than layer-wise,  supported by exisiting LTH.
why learn: customize to different local distributions, find local important parameters for personalization
automatically learn which parameters to adapt, 

In this paper, we aim to answer the research question: \textit{how to find the most important parameters for personalization on clients' local distribution?}

method 
Enlightened by LTH: there exists a  subnetwork that is crucial to the model performance (need rephrasing)
We believe that when personalizing a global model for each client, their also exists a subnetwork that is crucial for personalization. (We only need to adapt a subnetwork to personalize a global model to each local distribution.) 

a few sentence to introduce our algorithm

difference in 
goal: LTH aims to find a sparse network for efficiency, while we aim for better personalized model
method: LTH prunes the unimporant parameters  to zero value; while we set them as global aggregated value. 

Contribution
different types of distribution shifts, against multiple baselines, data size, 
Our visualization also verify that our algorithm successfully encode distribution information among clients. 




In this paper, we propose \textsc{{\algname}}, where we adapt both \textit{architecture and parameters} for each client to its local distribution during training. \bao{architecture may be confusing} Our method is based on the intuition that individual client models should select a necessary subset \chulin{personalized subset?} of shared parameters to encode personalized information for their local task. Our approach is inspired by the subnetwork discovery process used for the \textit{Lottery Ticket Hypothesis} \citep{frankle2019lottery}. The Lottery Ticket Hypothesis in its original form suggests that any neural network contains a significantly sparse subnetwork, called a ``lottery ticket network''. This subnetwork can be trained to achieve equivalent performance to its corresponding fully-trained network. Instead of pruning the "non-lottery ticket" parameters to zero, our method designates them instead for storing global information. This paper makes the following contributions:
\begin{itemize}
    \item We introduce a hypothesis for selecting parameters during training time for client personalization in FL.
    \item We propose \textsc{\algname}, a novel personalized FL algorithm based on our hypothesis, which is inspired by the iterative magnitude search procedure originally proposed for finding winning tickets via the Lottery Ticket Hypothesis \citep{frankle2019lottery}. To the best of our knowledge, this is the first algorithm to determine the model parameters for local personalization \textit{during FL}.
    \item We evaluate the performance of \textsc{\algname} across a range of benchmark datasets: CIFAR10 \citep{?}, CIFAR10-C \citep{?}, OfficeHome \citep{?}, and Tiny-ImageNet \citep{?}. We demonstrate superior performance across various distributional shifts that are common in real-world settings.
\end{itemize}

\section{Related Work}
\subsection{Federated Learning} 

\rt{Describe the prior methods in more detail}

There has been extensive work in federated learning on enhancing the training of a global model from various clients with non-independent and identically distributed (non-IID) data. Canonical approaches like FedAvg \cite{mcmahan2017} aims to develop a single global model that minimizes communication costs through local updates without requiring raw client data storage at a central server. However, challenges arise with non-IID data, leading to innovations in optimizing local learning algorithms through objective regularization \cite{acar2021federated}, local bias correction \cite{li2020federated}, and data handling techniques such as class-balanced resampling \cite{hsu2020federated} or loss reweighting \cite{wang2020addressing}. Different from these works, we adapt each client to its local data.

\subsection{Personalized Federated Learning} 

[Discuss differences in decoupling methods vs PMP framework vs LotteryFL]

Personalized federated learning aims to address the issue of data heterogeneity by adapting clients to their local data distribution. Common approaches include multitask learning \cite{Smith2017FederatedML, Agarwal2020FederatedRL}, clustering \cite{mansour2020approaches,Duan2021FlexibleCF, Ghosh2020AnEF}, transfer learning \cite{yu2022salvaging, zhao2018iid}, and meta learning \cite{jiang2023improving,fallah2020personalized,chen2019federated}. We focus on partial model personalization, which seeks to improve the performance of client models by altering a subset of their structure or weights to better suit their local tasks. It also addresses the issue of ``catastrophic forgetting'' \citep{McCloskey1989CatastrophicII}, an issue in personalized FL where global information is lost when fine-tuning a client model on its local distribution from a global initialization \citep{Kirkpatrick_2017, pillutla2022federated}. It does this by forcefully preserving a subset of parameters, $u$, to serve as a fixed global representation for all clients. However, existing methods introduced for partial model personalization \citep{pillutla2022federated, collins2021exploiting, xu2023personalized} require hand-selected partitioning of these shared and local parameters, and choose $u$ as only the input or output layers for their experiments. 

LotteryFL \citep{li2020lotteryfl} learns a shared global model via FedAvg \citep{mcmahan2017} and personalizes client models by pruning the global model via the vanilla LTH. Importantly, parameters are pruned to zero according to their magnitude after an iteration of batched stochastic gradient updates. However, due to a low final pruning percentage in LotteryFL, the lottery tickets found for each client share many of the same parameters, and lack sufficient personalization \citep{10.1007/978-3-031-19775-8_5}
